Improved Approximations for Multiprocessor Scheduling Under Uncertainty

This paper presents improved approximation algorithms for the problem of multiprocessor scheduling under uncertainty, or SUU, in which the execution of each job may fail probabilistically. This problem is motivated by the increasing use of distributed computing to handle large, computationally intensive tasks. In the SUU problem we are given n unit-length jobs and m machines, a directed acyclic graph G of precedence constraints among jobs, and unrelated failure probabilities q_{ij} for each job j when executed on machine i for a single timestep. Our goal is to find a schedule that minimizes the expected makespan, which is the expected time at which all jobs complete. Lin and Rajaraman gave the first approximations for this NP-hard problem for the special cases of independent jobs, precedence constraints forming disjoint chains, and precedence constraints forming trees. In this paper, we present asymptotically better approximation algorithms. In particular, we give an O(loglog min(m,n))-approximation for independent jobs (improving on the previously best O(log n)-approximation). We also give an O(log(n+m) loglog min(m,n))-approximation algorithm for precedence constraints that form disjoint chains (improving on the previously best O(log(n)log(m)log(n+m)/loglog(n+m))-approximation by a (log n/loglog n)^2 factor when n = poly(m). Our algorithm for precedence constraints forming chains can also be used as a component for precedence constraints forming trees, yielding a similar improvement over the previously best algorithms for trees.

==> lower.tex <==
\secput{lower}{Lin and Rajaraman's analysis is tight}
\note{Jacob: I think this should go as an appendix}
Lin and Ramarajan~\cite{LinRa07} give an $O(\log n)$-approximation
algorithm, called \LRind, for \suui.  In this section, we show that
the analysis is tight as long as $m = \Omega(\log n)$, where $m$ is
the number of machines and $n$ is the number of jobs.  Thus, a new
algorithm, and not just a tighter analysis, is necessary to get an
$o(\log n)$-approximation.

In each time step, the \LRind algorithm~\cite{LinRa07} considers the
success probabilities $p_{ij}=1-q_{ij}$ in nonincreasing order,
assigning machines to jobs as follows.  If machine $i$ is already
assigned to a job, consider the next $p_{ij}$.  Otherwise, if
$\sum_{x:\mbox{\scriptsize $x$ assigned to $j$}}p_{xj} + p_{ij} \leq
1$, assign $i$ to $j$.  That is, assign the machine to the job only if
it does not boost the sum of success probabilities for that job beyond~$1$.

\begin{theorem}
  For any positive integers $n$ of jobs and $m$ of machines, there
  exist success probabilities $p_{ij}$ such
  \begin{closeitemize}
  \item there exists a schedule with expected makespan $T$, and
  \item the expected makespan of \LRind is $\Omega(T
    \min\set{m,\log{n}})$.
  \end{closeitemize}
  \thmlabel{LRlower}
\end{theorem}
\begin{proof}
  Without loss of generality, we assume that $n$ is a power of $2$ and
  $\log n$ is even to simplify notation.  Also without loss of
  generality, we assume that whenever \LRind is presented with two
  identical probabilities, the adversary selects the order.  The proof
  generalizes by adjusting the probabilities by negligible values to
  force the choices.
  
  Let $r = \min\set{m,\log{n}/2}$.  Then we divide the $n$ jobs into
  $r+1$ groups $R,J_1,J_2,\ldots,J_r$, where $\card{J_k} = n/2^k$ for
  all $k$, and $\card{R} = n-\sum_{k=1}^r \card{J_k}$.\footnote{Group
    $R$ is just the remainder group so that sizes add to $n$---we
    include it for a complete description of the problem instance, but
    it has no real impact on the proof.}  We assign success
  probabilities $p_{ij}$ for job $j$ on machine $i$ as follows:
  \[
  p_{ij} = \left\{
    \begin{array} {r@{\quad:\quad}l}
      1/2^i & \mbox{if $i \leq r$, and $j \in J_k$ with $k \leq i$} \\
      1 & \mbox{if $i \leq r$, and $j \in R$} \\
      0 & \mbox{otherwise}
    \end{array} \right. \ .
  \]
  In other words, all jobs in group $J_k$ can run on only machines
  $k,k+1,\ldots r$.  If a job in $J_k$ can run on machine $i$, then the
  probability of success on that machine is $1/2^i$.  Jobs in group
  $R$ can run on all machines, and the probability of success is $1$. 
  
  We now describe a good way to schedule these jobs.  First schedule
  the jobs in $R$ across all $r$ viable machines until completions,
  taking $\ceil{\card{R}/r} < n$ steps.  Then assign all jobs in $J_i$
  to machine~$i$ in parallel, and run until completion.  The expected
  number of steps necessary to complete $J_i$ on machine~$i$ is
  $\card{J_i} 2^i = n$.  Since $\card{J_i} > \log n$ (and hence the
  expected number of successful runs is large) applying a Chernoff
  bound proves that the number of steps to complete $J_i$ on $i$ is
  $O(n)$ with high probability with respect to~$n$.  Taking a union
  bound over all $r\ll n$ implies that \emph{all} $J_i$ complete in
  $O(n)$ steps with high probability, and thus the total expected
  makespan of this schedule is $T = O(n)$.
  
  We now show that \LRind has expected makespan $\Omega(rn) =
  \Omega(rT)$ to complete the proof.  The jobs in $R$ have little
  effect, so let us ignore those.  \LRind may (under the
  adversarial-selection assumption) schedule jobs from $J_k$ only
  after \emph{all} jobs in lower groups have completed.  To simplify
  the proof, assume all jobs in $J_k$ complete instantaneously
  whenever fewer than $\log{n} > r$ jobs in $J_k$ remain.  Then the
  expected number of steps to complete all but $r$ jobs in $J_k$ is at
  least $(\card{J_k} - r)2^{k-1} > (\card{J_k}/2)2^{k-1} = \Omega(n)$.
  Thus, summing over all $r$ groups gives $\Omega(rn)$.
\end{proof}

This proof also implies that \LRind provides an $\Omega(\log
n)$-approximation to the deterministic problem of (obliviously)
scheduling the jobs such that every job attains at least a constant
probability of success.  Solving that deterministic problem directly,
however, does not yield any obvious improvement to the expected
makespan of the stochastic problem \suui.

